Particle creation in left-handed metamaterial transmission lines

Transmission lines are excellent examples of quantum simulators of quantum fields. By appropriately driving specific circuit elements, these devices can reproduce relativistic and quantum such as particle creation due to the non-adiabatic stimulation of the quantum vacuum. We investigate particle creation in left-handed transmission lines induced by the modulation of the Josephson energy in superconducting quantum interference devices. Our results show that, as a consequence of the peculiar dispersion relations present in these systems, particle production occurs with much more favorable conditions with respect to the usual right-handed transmission lines.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
